Hoeffding adaptive trees for multi-label classification on data streams

Data stream learning is a very relevant paradigm because of the increasing real-world scenarios generating data at high velocities and in unbounded sequences. Stream learning aims at developing models that can process instances as they arrive, so models constantly adapt to new concepts and the temporal evolution in the stream. In multi-label data stream environments where instances have the peculiarity of belonging simultaneously to more than one class, the problem becomes even more complex and poses unique challenges such as different concept drifts impacting different labels at simultaneous or distinct times, higher class imbalance, or new labels emerging in the stream. This paper proposes a novel approach to multi-label data stream classification called Multi-Label Hoeffding Adaptive Tree (MLHAT). MLHAT leverages the Hoeffding adaptive tree to address these challenges by considering possible relations and label co-occurrences in the partitioning process of the decision tree, dynamically adapting the learner in each leaf node of the tree, and implementing a concept drift detector that can quickly detect and replace tree branches that are no longer performing well. The proposed approach is compared with other 18 online multi-label classifiers on 41 datasets. The results, validated with statistical analysis, show that MLHAT outperforms other state-of-the-art approaches in 12 well-known multi-label metrics.

==> 4_experimental.tex <==
\section{Experimental study}\label{sec:exp}

This section presents the experimental study and comparison with the state-of-the-art works. The experiments are designed to answer the following research questions:
\begin{itemize}
    \item \textbf{RQ1:} Can \ac{MLHAT} demonstrate competitive performance compared to the state of the art incremental decision tree methods for multi-label data streams?
    \item \textbf{RQ2:} Is it more beneficial to use \ac{MLHAT}'s native multi-label split criterion rather than applying \acf{PT} to use a non-adapted split criterion?
    %\item \textbf{RQ3:} Does the performance of \ac{MLHAT} improve when introduced in ensemble-type models with respect to the state of the art in this field? 
    \item \textbf{RQ3:} Is \ac{MLHAT} robust in a multi-label data stream scenario where concept drift may appear?
\end{itemize}



\subsection{Experimental setup}


\subsubsection{Algorithms}

Table \ref{tab:algorithms} presents a taxonomy of the 16 multi-label incremental algorithms used in this experimental study, including \acf{BR} to transform the problem and \acf{AA} methods, as well as whether they are adaptable to concept drift. All algorithms are implemented in Python and are publicly available in the River library \cite{Montiel2021}. The source code of \acs{MLHAT} is publicly available in the repository associated with this work\footnote{\url{https://github.com/aestebant/mlhat}} for the sake of reproducibility. In model selection, approaches based on \ac{IDT} have special prevalence. Thus, we consider 5 multi-class \acp{IDT} transformed to \ac{MLC} using \ac{BR}; 3 \acp{IDT} for \ac{MLC}, and 2 forest-based methods, i.e., ensembles designed for specific trees as base models. Moreover, the experimentation includes other algorithms from well-known paradigms like neighbors, rules, Bayes, and bagging and boosting, as well as the recent \acs{MLBELS}, based on neural network and trained in mini-batches \cite{Bakhshi2024}. In this last case, in order to make the experimentation conditions as similar as possible to the other proposals, which work purely online, the smallest batch size studied by the authors, 50 instances, is used.
In general, the hyperparameter setting has followed three principles: (i) not to make individualized adjustments per dataset, (ii) to start from the configurations suggested by the authors or mostly used in the literature, and (iii) to keep equivalent configurations in models of the same family. Thus, all Hoeffding trees, including our \acs{MLHAT}, have been configured with Hoeffding significance $\delta_{spl}=1\mathrm{e}{-5}$ and a grace period of $\kappa_{spl}=200$, and all ensembles have been configured with 10 base models. The complete parameter specification per algorithm can be found in the associated repository.


\begin{table}[h]
    \centering
    \caption{Algorithms included in the comparative studies}\label{tab:algorithms}
    \begin{tblr}{
        width=\linewidth,
        colspec={Q[l,m] Q[c,m] Q[l,m] X[l,m] X[0.4,c,m]},
        colsep=2pt,
        rowsep=0.2pt,
        row{1-Z}={font=\scriptsize}
    }
    \toprule
    Family & Ref & Acr & Algorithm & {Concept-drift\\adaptable}\\
    \midrule
    BR+IDT & \cite{Domingos2000} & \acs{HT} & \acl{HT} & \ding{53}\\
    BR+IDT & \cite{Bifet2009} & \acs{HAT} & \acl{HAT} & \ding{51}\\
    BR+IDT & \cite{Manapragada2018} & \acs{EFDT} & \acl{EFDT} & \ding{53}\\
    BR+IDT & \cite{Gouk2019} & \acs{SGT} & \acl{SGT} & \ding{53}\\
    BR+IDT & \cite{Mourtada2021} & \acs{MT} & \acl{MT} & \ding{53}\\
    
    {BR+\\Bayesian} & \cite{Bifet2009a} & \acs{NB} & \acl{NB} & \ding{53}\\
    {BR+\\Distance} & \cite{Montiel2021} & \acs{kNN} & \acl{kNN} & \ding{53}\\
    BR+Rules & \cite{Duarte2016} & \acs{AMR} & \acl{AMR} & \ding{51}\\
    
    %BR+Ensb & \cite{Oza2001} & \acs{OB} & \acl{OB}\\
    BR+Ensb & \cite{Bifet2009a} & \acs{ABA} & \acl{ABA} + \acl{LR} & \ding{51}\\
    %BR+Ensb & \cite{Oza2001} & \acs{OBO} & \acl{OBO}\\
    BR+Ensb & \cite{Bifet2009a} & \acs{ABO} & \acl{ABO} + \acl{LR} & \ding{51}\\
    %BR+Ensb & \cite{Bifet2010} & \acs{LB} & \acl{LB}\\
    %BR+Ensb & \cite{DeBarros2016} & \acs{BOLE} & \acl{BOLE}\\
    
    %BR+Ensb+DT & \cite{Montiel2021} & \acs{OBHT} & \acl{OBHT}\\
    %BR+Ensb+DT & \cite{Montiel2021} & \acs{OBHAT} & \acl{OBHAT}\\
    %BR+Ensb+DT & \cite{Montiel2021} & \acs{OBEFDT} & \acl{OBEFDT}\\
    %BR+Ensb+DT & \cite{Gomes2019} & \acs{SRPHAT} & \acl{SRPHAT}\\
    
    BR+Forest & \cite{Gomes2017} & \acs{ARF} & \acl{ARF} & \ding{51}\\
    BR+Forest & \cite{Mourtada2021} & \acs{AMF} & \acl{AMF} & \ding{53}\\
    
    AA+IDT & \cite{Read2012} & \acs{MLHT} & \acl{MLHT} & \ding{53}\\
    AA+IDT & \cite{Read2012} & \acs{MLHTPS} & \acl{MLHTPS} & \ding{53}\\
    AA+IDT & \cite{Osojnik2017} & \acs{iSOUPT} & \acl{iSOUPT} & \ding{53}\\
    AA+NN & \cite{Bakhshi2024} & \acs{MLBELS} & \acl{MLBELS} & \ding{53}\\
    
    %AA+Ensb+DT & \cite{Read2012}  & \acs{OBMLHTPS} & \acl{OBMLHTPS}\\
    %AA+Ensb+DT & \cite{Osojnik2017}  & \acs{SRPMLHTPS} & \acl{SRPMLHTPS}\\
    %AA+Ensb+DT & \cite{Read2012} & \acs{OBiSOUPT} & \acl{OBiSOUPT}\\
    %AA+Ensb+DT & \cite{Osojnik2017} & \acs{SRPiSOUPT} & \acl{SRPiSOUPT}\\
    
    AA+IDT & This & \acs{MLHAT} & \acl{MLHAT} & \ding{51}\\
    %AA+Ensb+DT & - & \acs{OBMLHAT} & \acl{OBMLHAT}\\
    %AA+Ensb+DT & - & \acs{SRPMLHAT} & \acl{SRPMLHAT}\\
    \bottomrule
    \end{tblr}
\end{table}




\subsubsection{Datasets}

Multi-label datasets used in the experimental study cover a wide range of properties. On the one hand, we evaluate the performance of the algorithms included in the study on 29 real datasets publicly available\footnote{\url{https://www.uco.es/kdis/mllresources/}} of up to 269,648 instances, 31,802 features, and 374 labels. The complete specification of each dataset is shown in Table \ref{tab:datasets} attending to the number of instances, features, and labels, as well as other statistics like cardinality (average amount of labels per instance) and density (cardinality divided by the number of labels). Moreover, the last column indicates whether the instances in the dataset are presented in a temporal order: yes (\ding{51}), no (\ding{53}), or this information can not be known from the provided description (-). Since in these datasets there is no explicit information about concept drift, this factor can give an idea about the chances of finding concept drift in them.

\begin{table}[htb]
    \centering
    \caption{Real-world datasets used in the experimental study}\label{tab:datasets}
    \begin{tblr}{
        width=\linewidth,
        colspec={X[l,m] *{5}{Q[r,m]} X[0.7,c,m]},
        colsep=2pt,
        rowsep=0.2pt,
        row{1-Z}={font=\scriptsize}
    }
    \toprule
    Dataset & Instan. & Features & Labels & Card. & Dens. & Temporal order\\
    \midrule
    Flags  & 194 & 19 & 7 & 3.39 & 0.48 & \ding{53} \\
    %Chd  & 555 & 49 & 6 & 2.58 & 0.43  \\
    WaterQuality  & 1,060 & 16 & 14 & 5.07 & 0.36 & - \\
    Emotions  & 593 & 72 & 6 & 1.87 & 0.31 & \ding{53} \\
    VirusGO  & 207 & 749 & 6 & 1.22 & 0.20 & \ding{53} \\
    Birds  & 645 & 260 & 19 & 1.01 & 0.05 & - \\
    Yeast  & 2,417 & 103 & 14 & 4.24 & 0.30 & \ding{53} \\
    Scene  & 2,407 & 294 & 6 & 1.07 & 0.18 & \ding{53} \\
    Gnegative  & 1,392 & 440 & 8 & 1.05 & 0.13 & - \\
    Plant  & 978 & 440 & 12 & 1.08 & 0.09 & - \\
    %Cal500  & 502 & 68 & 174 & 26.04 & 0.15  \\
    Human  & 3,106 & 440 & 14 & 1.19 & 0.08 & - \\
    %Genbase  & 662 & 1,186 & 27 & 1.25 & 0.05  \\
    Yelp  & 10,806 & 671 & 5 & 1.64 & 0.33 & \ding{51} \\
    Medical  & 978 & 1,449 & 45 & 1.25 & 0.03 & \ding{51} \\
    Eukaryote  & 7,766 & 440 & 22 & 1.15 & 0.05 & - \\
    Slashdot  & 3,782 & 1,079 & 22 & 1.18 & 0.05 & \ding{51} \\
    Enron  & 1,702 & 1,001 & 53 & 4.27 & 0.08 & \ding{51} \\
    Hypercube  & 100,000 & 100 & 10 & 1.00 & 0.10 & - \\
    %Hypersphere  & 100,000 & 100 & 10 & 2.31 & 0.23  \\
    Langlog  & 1,460 & 1,004 & 75 & 15.94 & 0.21 & \ding{51} \\
    Stackex  & 1,675 & 585 & 227 & 2.41 & 0.01 & \ding{51} \\
    Tmc  & 28,596 & 500 & 22 & 2.22 & 0.10 & \ding{51} \\
    Ohsumed  & 13,929 & 1,002 & 23 & 0.81 & 0.04 & \ding{51} \\
    D20ng  & 19,300 & 1,006 & 20 & 1.42 & 0.07 & \ding{51} \\
    Mediamill  & 43,907 & 120 & 101 & 4.38 & 0.04 & - \\
    %Corel5k  & 5,000 & 499 & 374 & 3.52 & 0.01  \\
    Corel16k  & 13,766 & 500 & 153 & 2.86 & 0.02 & \ding{53} \\
    Bibtex & 7,395 & 1,836 & 159 & 2.40 & 0.02 & \ding{53} \\
    Nuswidec & 269,648 & 129 & 81 & 1.87 & 0.02 & - \\
    Nuswideb & 269,648 & 501 & 81 & 1.87 & 0.02 & -  \\
    Imdb  & 120,919 & 1,001 & 28 & 1.00 & 0.04 & \ding{53}  \\
    YahooSociety  & 14,512 & 31,802 & 27 & 1.67 & 0.06 & - \\
    Eurlex  & 19,348 & 5,000 & 201 & 2.21 & 0.01 & \ding{51} \\
    \bottomrule
    \end{tblr}
\end{table}

To the authors' knowledge, there are no public multi-label datasets that expressly contain information about concept-drift \cite{Read2012, Shi2014,Cerri2021}. To address this issue, 12 additional datasets are generated synthetically to study the impact of different types of concept drift. These datasets have been generated with the MOA framework \cite{Bifet2010a} and are public in the repository associated to this paper. We employ three multi-label generators based on Random Tree, \ac{RBF} and Hyper-plane, under two configurations widely used \cite{Read2012}: 30 attributes and 8 labels, and 80 attributes and 25 labels. The drifts are controlled by two parameters: the label cardinality $Z$ and the label dependency $u$, that are altered in different ways to generate the four main types of concept drift in \ac{MLC}: sudden, gradual, incremental and recurrent. In all cases, the drifts take place at 3 times depending on the size $N$ of the stream: at times $N/4$, $2N/4$ and $3N/4$, and each drift changes the underlying concept of the stream. Thus, the controlled parameters in the first stretch of the stream are $Z=1.5$, $u=0.25$; in the second only the label dependency changes, so we have $Z=1.5$, $u=0.15$; in the third stretch only the cardinality changes to have $Z=3.0$, $u=0.15$; and finally, in the fourth, they both change to end up with $Z=1.5$, $u=0.25$ again. In the recurrent case, only the configurations of the 1st and 3rd stretches are alternated twice. Table \ref{tab:datasets-synth} shows the main characteristics of these synthetic datasets regarding features, labels, type of concept drift and its width, i.e., for how many instances the drift change extends. For more details, refer to the paper repository.

\begin{table*}[t]
    \centering
    \caption{Synthetic datasets used in the experimental study}\label{tab:datasets-synth}
    \begin{tblr}{
        width=0.7\linewidth,
        colspec={X[l,m] *{6}{Q[c,m]}},
        colsep=2pt,
        rowsep=0.2pt,
        row{1-Z}={font=\scriptsize}
    }
    \toprule
    Dataset & Instances & Features & Labels & Generator & Drift type & Drift width\\
    \midrule
    SynTreeSud & 50,000 & 20 num.+10 cat. & 8 & Random Tree & sudden & 1\\
    SynRBFSud & 50,000 & 80 numeric & 25 & Random RBF & sudden & 1\\
    SynHPSud & 50,000 & 30 numeric & 8 & Hyper Plane & sudden & 1\\
    SynTreeGrad & 50,000 & 20 num.+10 cat. & 8 & Random Tree & gradual & 500\\
    SynRBFGrad & 50,000 & 80 numeric & 25 & Random RBF & gradual & 500\\
    SynHPGrad & 50,000 & 30 numeric & 8 & Hyper Plane & gradual & 500\\
    SynTreeInc & 50,000 & 20 num.+10 cat. & 8 & Random Tree & incremental & 275\\
    SynRBFInc & 50,000 & 80 numeric & 25 & Random RBF & incremental & 275\\
    SynHPInc & 50,000 & 30 numeric & 8 & Hyper Plane & incremental & 275\\
    SynTreeRec & 50,000 & 20 num.+10 cat. & 8 & Random Tree & recurrent & 1\\
    SynRBFRec & 50,000 & 80 numeric & 25 & Random RBF & recurrent & 1\\
    SynHPRec & 50,000 & 30 numeric & 8 & Hyper Plane & recurrent & 1\\
    \bottomrule
    \end{tblr}
\end{table*}



\subsubsection{Evaluation metrics}\label{sec:evaluation}

Due to the incremental nature of the data streams, the canonical way to evaluate performance working with them follows a test-then-train scheme known as prequential evaluation \cite{Gama2009}. In this work, we apply this methodology for all the experiments setting a forgetting factor of $\alpha=0.995$ and 50 steps between evaluations.

For comparing the performance between algorithms, we employ 11 different metrics that evaluate the total and partial correctness of multi-label prediction \cite{Bogatinovski2022}, as well as the total computing time in seconds. The metrics are defined as follows over $L$ labels and $n$ instances.

Example-based metrics evaluate the difference between the actual and predicted labelsets, averaged over $n$. Given a true labelset $Y_i = \{y_{i1}...y_{i L}\}$ and a predicted one $Z_i = \{ z_{i1}...z_{i L} \}$, the example-based metrics considered are:
\begin{equation}
    \begin{split}
    &\text{\footnotesize Subset accuracy} = \frac{1}{n}\sum^n_{i=0} 1 | Y_i = Z_i \\
    &\text{\footnotesize Hamming loss} = \frac{1}{n L} \sum^n_{i=0} \sum^L_{l=0} 1 | y_{il} \neq z_{il} \\
    %\text{Example-based accuracy} &= \frac{1}{n} \sum^n_{i=0} \frac{|Y_i \cap Z_i|}{|Y_i \cup Z_i|} \\
    &\text{\footnotesize Example-based precision} = \frac{1}{n} \sum^n_{i=0} \frac{|Y_i \cup Z_i|}{|Z_i|} \\
    &\text{\footnotesize Example-based recall} = \frac{1}{n} \sum^n_{i=0} \frac{|Y_i \cup Z_i|}{|Y_i|} \\
    &\text{\footnotesize Example-based F1} = \frac{1}{n} \sum^n_{i=0} \frac{2 |Y_i \cup Z_i|}{|Y_i| + |Z_i|}
    \end{split}
\end{equation}

Label-based metrics measure the performance across the different labels, that can be micro- or macro-averaged depending on if it is used the joint statistics for all labels or the per-label measures are averaged into a single value. Given for each label $l$ its true positives $tp_l = \sum^n_{i=0} 1 | y_{il} = z_{il} = 1$, true negatives $tn_l = \sum^n_{i=0} 1 | y_{il} = z_{il} = 0$, false positives $fp_l = \sum^n_{i=0} 1 | y_{il}=0, z_{il}=1$, and false negatives $fn_l = \sum^n_{i=0} 1 | y_{il}=1, z_{il}=0$, the macro-averaged metrics considered are:
\begin{equation}
\begin{split}
    &\text{\footnotesize Macro-averaged precision} = \frac{1}{L} \sum^L_{l=0} \frac{tp_l}{tp_l + fp_l}\\
    &\text{\footnotesize Macro-averaged recall} = \frac{1}{L} \sum^L_{l=0} \frac{tp_l}{tp_l + fn_l}
\end{split}
\end{equation}
while the considered micro-averaged metrics are defined as:
\begin{equation}
\begin{split}
&\text{\footnotesize Micro-averaged precision} = \frac{\sum^L_{l=0} tp_l}{\sum^L_{l=0} tp_l + \sum^L_{l=0} fp_l}\\
&\text{\footnotesize Micro-averaged recall} = \frac{\sum^L_{l=0} tp_l}{\sum^L_{l=0} tp_l + \sum^L_{l=0} fn_l}
\end{split}
\end{equation}

Additionally, Macro-averaged F1 and Micro-averaged F1 are also considered, defined as the harmonic mean of precision and recall in an equivalent way to the example-based F1 defined above.



\subsection{Analysis of components in MLHAT}\label{sec:optimization}

As discussed in the model description in Section \ref{sec:proposal}, \ac{MLHAT} is highly configurable through a wide variety of hyperparameters ranging from the entropy and cardinality thresholds to the classifiers to be used in the leaves and the metrics to be used to monitor the concept drift. The configuration of these hyperparameters is non-trivial, as it encompasses a multitude of possible combinations that evolve categorical, integer, decimal, and logarithmic parameters. In response to this challenge, we employ a well-known systematic approach for hyperparameter optimization \cite{Bischl2023} that combines the \ac{TPE} algorithm to generate configurations that maximize the objective function, with the Hyperband pruner that accelerates the search by discarding the less promising combinations. This methodology allows us to efficiently traverse the vast hyperparameter space of \ac{MLHAT}, as well as to understand the importance of each hyperparameter and its influence on the final performance. The study has been implemented in Python through the Optuna framework \cite{Akiba2019}.

\begin{table*}[htb]
    \centering
    \caption{Hyperparameter study for MLHAT}\label{tab:hyperparams}
    \begin{tblr}{
        width=.8\linewidth,
        colspec={Q[l,m] X[l,m] Q[c,m]},
        colsep=3pt,
        rowsep=1pt,
        row{1-Z}={font=\scriptsize},
    }
    \toprule
    Parameter & Studied values & Final Value\\
    \midrule
    Significance for split $\delta_{spl}$ & Fixed by state-of-the-art & 1e-5\\
    Leaf grace period $\kappa_{spl}$ & Fixed by state of the art & 200\\
    Significance for tree replacement $\delta_{alt}$ & [0.01, 0.10] & 0.05 \\
    Alternate tree grace period. $\kappa_{alt}$ & [100, 500] & 300\\
    Cardinalty threshold $\eta$ & [100, 1000] & 620\\
    Poisson parameter $\lambda$ & [1, 6] & 1\\
    Drift metric $e$ & Subset Acc., Hamming loss, Micro-F1, Macro-F1 & Hamming loss\\
    $\gamma_{\downarrow C}$ base & \acs{HT}, \acs{kNN}, \acs{NB}, \acs{LR}  & \acs{kNN}\\
    $\gamma_{\downarrow C}$ transformation & \acs{BR}, \acs{LP}, \acs{CC} & \acs{LP}\\
    $\gamma_{\uparrow C}$ base & \acs{NB}, \acs{LR} & \acs{LR}\\
    $\gamma_{\uparrow C}$ ensemble & \acs{BA} \cite{Oza2001}, \acs{BO} \cite{Oza2001}, \acs{BOLE} \cite{DeBarros2016}, \acs{SRP} \cite{Gomes2019} & \acs{BA}\\
    $\gamma_{\uparrow C}$ transformation & \acs{BR}, \acs{LP}, \acs{CC} & \acs{BR}\\
    \bottomrule
    \end{tblr}
\end{table*}

The conditions of the study are mainly given by the optimization function and the range in which each hyperparameter will move. The optimization function has been defined as the Subset accuracy by means of the prequential evaluation (see Section \ref{sec:evaluation}) of a minimum subset of the datasets included in the experimentation, selected among the less complex ones, to make the iterative search feasible, and maximizing the differences between them in terms of cardinality, density, and concept drift. Specifically, datasets \textit{Flags}, \textit{Emotions}, \textit{VirusGO}, \textit{Birds}, \textit{Yeast}, \textit{Scene}, \textit{SynHPSud}, and \textit{SynHPGrad} are selected (see Tables \ref{tab:datasets} and \ref{tab:datasets-synth}), i.e. 19\% of the total set of datasets included in the experiment. The search ranges per hyperparameter are shown in Table \ref{tab:hyperparams}. For the numerical attributes, typical ranges from the literature on Hoeffding trees have been used. To monitor concept drift, any \ac{MLC} metric can be used, although it is desirable that it covers overall performance and is sensitive to class imbalance, since it is going to work at the level of each node of the tree. Thus, in this study, two example metrics and two label metrics are tested. Any pair of online multi-label classifiers can be used in the leaves taking into account that (i) they must not incorporate drift detection mechanisms, since this is done at tree level, and (ii) a balance between short and long-term performance is desirable to cover the possible scenarios that a leaf may face, as discussed in Section \ref{sec:leaves}. For the low complexity classifier, we study a representation of the four main paradigms in online classification: decision trees, distance-based models, Naïve Bayes and linear models. For the high complexity classifier, we compare different ensembles and using low complexity methods as the base model to maintain the complexity of the model under control. In all cases, the ensembles work with 10 base models, as usual in the online learning paradigm \cite{Alberghini2022}. In both low- and high-complexity classifiers different transformations to pass from the multi-label space to a single-label space are studied.

\begin{figure*}[htb]
    \centering
    \subfloat[Optimization history]{\includegraphics[width=.4\linewidth]{figs/optimization_hist.pdf}}\quad
    \subfloat[Hyperparameter importance according functional ANOVA]{\includegraphics[width=.4\linewidth]{figs/params_importance.pdf}}\\
    \subfloat[Parallel coordinate plot with the most influential parameters. Some parameters have been omitted for visual clarity as they do not have a sufficiently meaningful range of variability.]{\includegraphics[width=.8\linewidth]{figs/parallel_coordinates.pdf}}
    \caption{Automatic optimization of MLHAT}
    \label{fig:hyperparams-study}
\end{figure*}

Figure \ref{fig:hyperparams-study} shows the results of the hyperparameters search, including the optimization history obtained with the framework described above, and the importance of each hyperparameter in the final performance according to the  ANOVA functional framework \cite{Hutter2014}, that quantifies the influence of both single hyperparameters and the interactions between them from the marginal predicted performance. Finally, the parallel coordinate plot shows the most promising hyperparameter combination based on  the average performance in the subset of datasets selected for this phase. Please note that not all combinations are present because of the guided search method employed. The best hyperparameter configuration found by the optimization method is shown in the last column of Table \ref{tab:hyperparams}. This configuration will be used in the rest of the experimental study over the whole set of datasets.

The study indicates that the high-complexity classifier is the most relevant parameter for \ac{MLHAT} performance, specifically the label transformation method, where \ac{BR} performs much better than \ac{LP} and \ac{CC}, probably because it deals more efficiently with label imbalance. In contrast, the transformation used in the low-complexity classifier does not have very important differences in the final result: when working with little data, the multi-label space is small and the three studied methods provide equivalent results. The second most important parameter is the threshold for establishing a high-cardinality scenario. Although the results will vary depending on the pair of classifiers used, it appears that around 600 instances received at a leaf node is the optimal point to move to the most complex classifier. When dealing with the highly complex scenario, it becomes evident that bagging-based ensembles, represented by \ac{BA} and \ac{SRP}, offer more advantages compared to boosting-based ensembles, namely \ac{BO} and \ac{BOLE}. This observation arises from the fact that boosting primarily concentrates on enhancing the performance of misclassified instances. However, in the context of \ac{MLHAT}, where the feature space has already undergone discrimination through the tree structure, this boosting emphasis may result in overfitting. As a base classifier, \ac{LR} far outperforms \ac{NB}, which, having not completed any runs because they were pruned earlier, does not appear in the graph. In the low complexity case, working with a single model and not an ensemble, it is required a more sophisticated learner to obtain good results. Thus, \ac{HT} and \ac{kNN} are the most promising. Finally, attending to the metric for monitoring concept drift, although not as influential as other parameters, there is a clear loser: macro-average is not a good approach, as it does not take into account label imbalance. The rest of the metrics have a similar potential to detect concept drift in general, although probably in studies where only a specific type of concept drift is affected, one metric would respond better than another to accelerate detection. The final configuration for \ac{MLHAT}, showed in Table \ref{tab:hyperparams}, follows these lines: for the low complexity leaf classifier a multi-label \ac{kNN} obtains better performance than the closest alternative of \ac{HT}. The \ac{LP} transformation is preferred due to the possibility to capture better the label correlation than \ac{BR}. The high complexity classifier is conformed as a bagging of \acp{LR}, that combines good performance and fast execution in data-intense scenarios. Hamming loss is the metric selected for monitoring the concept drift, showing that is desirable an example-based approach and to use a metric that keeps a balance between the proportion of correct and incorrect labels inside the labelset, rather than the subset accuracy, that is too strict to be informative. With this configuration, 620 instances is the optimal threshold a leaf should see to pass from the low to the high cardinality scenarios, and 450 are the minimal instances an alternate tree should see to try to replace the main one. Finally, the $Poisson(\lambda=1)$ indicates that is desirable to model the instances' weight as events that occur relatively infrequently but with a consistent average rate.


\begin{figure*}[htb]
    \centering
    \includegraphics[width=.8\linewidth]{figs/paper_combining_effect.pdf}
    \caption{Effect on the performance of combining predictions from the main and the alternate trees in \ac{MLHAT}}
    \label{fig:combpred}
\end{figure*}

Once the \ac{MLHAT} hyperparameters have been established, the last study examines the effect of combining the predictions of the alternate trees that are constructed during the occurrence of concept-changes explained in Section \ref{sec:classification}. This study focuses on the micro-average F1 score obtained with the fixed parameters of Table \ref{tab:hyperparams} and altering only the way of obtaining the predictions during the prequential evaluation. Figure \ref{fig:combpred} shows the differences between results per dataset. Combining the predictions gives an average F1 score of 0.4916, while using the main tree alone gives 0.4475. In other words, the method proposed in Section \ref{sec:proposal} improves the results on average by 5\%. The results per dataset will depend on whether \ac{MLHAT} detects the concept drift alarm and whether it is finally confirmed or not. In most datasets, this measure has little effect because either the concept drift does not occur or it is quickly confirmed and the alternate structure becomes part of the main tree. In any case, since the grace period $\kappa_{alt}$ must be exceeded to consider the predictions of the alternate trees, and the predictions are weighted with the branch error in real time, the inclusion of the possible alternate trees is done in a fairly conservative manner that prevents it from having significant adverse effects. Moreover, we see datasets such as \textit{D20ng}, \textit{Nuwideb} or synthetic datasets with explicit concept drift information where combining the predictions has a very positive effect on the average result, with differences of up to 30 tenths in F1. This is due to the fact that in these cases there are more gradual concept drifts in which it is positive to consider at the same time the main tree and the alternatively emerging branches. In conclusion, this measure is considered positive for the overall performance of MLHAT and will be used in the remainder of the comparative study.


\subsection{Analysis of MLHAT compared to previous proposals}\label{sec:overallperf}

This section evaluates and compares the overall performance of the 17 online algorithms in the 41 datasets for the 11 \ac{MLC} metrics, plus time of execution, to address RQ1. Table \ref{tab:singleresults} shows a summary of the results by averaging the measures for all the datasets, while Table \ref{tab:friedmansingle} shows the rankings and their associated $p$-value according to Friedman statistic test \cite{Dietterich1998}. The complete results are available in the repository\footnote{\url{https://github.com/aestebant/mlhat}}. Friedman tests show that there are significant differences with high confidence ($p\mathrm{-value} \rightarrow 0$) for all metrics. Therefore, the post-hoc Bonferroni-Dunn procedure \cite{Dietterich1998} is applied on a selection of the most representative metrics to find between which groups of algorithms these differences occur. Figure \ref{fig:post-hoc} shows the results at confidence level $\alpha=99\%$ for subset accuracy, hamming loss, example-based F1, micro-averaged F1, macro-averaged F1, and time.


\begin{table*}[htb]
    \centering
    \caption{Average results for each evaluation metric considering all datasets}\label{tab:singleresults}
 %  \caption{Performance of 12 metrics averaging the measures for all the datasets}\label{tab:singleresults}
    \begin{tblr}{
        width=.95\linewidth,
        colspec={X[l,m] *{12}{Q[r,m]}},
        colsep=3pt,
        rowsep=-1pt,
        row{1-Z}={font=\scriptsize}
    }
\toprule
Algorithm & Su. Acc & H. Loss & Ex. F1 & Ex. Pre & Ex. Rec & Mi. F1 & Mi. Pre & Mi. Rec & Ma. F1 & Ma. Pre & Ma. Rec & Time (s)\\
\midrule
MLHAT &      \textbf{0.2646} &   0.1301 &      \textbf{0.4755} &        0.6195 &       0.4892 &    \textbf{0.4855} &      0.5309 &     0.4556 &    \textbf{0.3871} &      0.4691 &     \textbf{0.3661} &  14994\\
KNN &      0.2018 &   0.1273 &      0.3321 &        0.4781 &       0.3234 &    0.3744 &      0.5170 &     0.3220 &    0.2609 &      0.4035 &     0.2309 & 102362\\
NB &      0.0993 &   0.1842 &      0.2338 &        0.3794 &       0.3157 &    0.2479 &      0.3392 &     0.3211 &    0.1754 &      0.2198 &     0.2582 &   7578\\
AMR &      0.2111 &   0.1177 &      0.3343 &        0.5716 &       0.3263 &    0.3728 &      0.6513 &     0.3207 &    0.2626 &      0.4467 &     0.2356 &  29882\\
HT &      0.1512 &   0.1232 &      0.2687 &        0.5127 &       0.2608 &    0.3176 &      0.5336 &     0.2574 &    0.2003 &      0.3424 &     0.1770 &  42975\\
HAT &      0.1746 &   0.1195 &      0.3076 &        0.5352 &       0.3008 &    0.3612 &      0.5494 &     0.2972 &    0.2319 &      0.3659 &     0.2056 &  43651\\
EFDT &      0.1620 &   0.1236 &      0.3066 &        0.4996 &       0.3028 &    0.3603 &      0.5095 &     0.3015 &    0.2413 &      0.3465 &     0.2138 &  36942\\
SGT* &      0.0337 &   0.2562 &      0.1221 &        0.4381 &       0.2103 &    0.1392 &      0.2115 &     0.2122 &    0.1016 &      0.1638 &     0.1991 & 298466\\
MT* &      0.1224 &   0.1285 &      0.1920 &        0.5126 &       0.1789 &    0.2223 &      0.5606 &     0.1750 &    0.1335 &      0.2922 &     0.1232 & 186185\\
ARF &      0.1967 &   \textbf{0.1126} &      0.3178 &        0.5507 &       0.3008 &    0.3730 &      0.6886 &     0.2972 &    0.2440 &      0.4710 &     0.2081 &  29308\\
AMF* &      0.1935 &   0.1247 &      0.2987 &        \textbf{0.6457} &       0.2834 &    0.3367 &      0.6681 &     0.2790 &    0.2267 &      0.4547 &     0.2029 & 131491\\
ABALR &      0.2189 &   0.1156 &      0.3283 &        0.5958 &       0.3178 &    0.3638 &      \textbf{0.7057} &     0.3113 &    0.2509 &      \textbf{0.4808} &     0.2254 &  12584\\
ABOLR &      0.2162 &   0.1164 &      0.3276 &        0.5931 &       0.3182 &    0.3616 &      0.6959 &     0.3115 &    0.2512 &      0.4682 &     0.2270 &  13868\\
MLBELS* &      0.2046 &   0.1858 &      0.4595 &        0.4854 &       \textbf{0.5452} &    0.4703 &      0.4579 &     \textbf{0.5173} &    0.3090 &      0.4518 &     0.3650 &  77813\\
MLHT &      0.1419 &   0.1723 &      0.2495 &        0.2792 &       0.2419 &    0.2523 &      0.2992 &     0.2343 &    0.1139 &      0.2497 &     0.1522 &   \textbf{1458}\\
MLHTPS &      0.1211 &   0.1343 &      0.1900 &        0.4596 &       0.1856 &    0.2096 &      0.4164 &     0.1823 &    0.1337 &      0.3058 &     0.1327 &  29517\\
iSOUPT &      0.2154 &   0.1175 &      0.3284 &        0.5938 &       0.3202 &    0.3710 &      0.6908 &     0.3149 &    0.2507 &      0.4608 &     0.2247 &   6486\\
\bottomrule
\SetCell[c=13]{l} Best results are in bold.\\
\SetCell[c=13]{l,m,.9\linewidth} * Results computed without considering all datasets due to scalability limitations. The physical limitations for all the experiments are set to 200GB of RAM and 240 hours of executions.\\
    \end{tblr}
\end{table*}


\begin{table*}[htb]
    \centering
    \caption{Friedman's test and average ranks for each evaluation metric}\label{tab:friedmansingle} 
    %\caption{Friedman's  average ranks for multi-label metrics across all datasets}\label{tab:friedmansingle}
    \begin{tblr}{
        width=.9\linewidth,
        colspec={X[l,m] *{12}{Q[r,m]}},
        colsep=2pt,
        rowsep=-1pt,
        row{1-Z}={font=\scriptsize},
    }
\toprule
Algorithm & Su.Acc & H.Loss & Ex.F1 & Ex.Pre & Ex.Rec & Mi.F1 & Mi.Prec & Mi.Rec & Ma.F1 & Ma.Prec & Ma.Rec & Time (s) \\
\midrule
MLHAT & \textbf{4.000} & 9.024 & \textbf{3.024} & 6.878 & \textbf{2.902} & \textbf{3.439} & 9.415 & \textbf{3.098} & \textbf{2.463} & 6.341 & \textbf{2.659} & 7.049 \\ 
KNN & 5.463 & 9.439 & 7.049 & 9.585 & 7.585 & 6.878 & 9.780 & 7.512 & 6.415 & 7.268 & 7.293 & 13.488 \\ 
NB & 12.512 & 12.573 & 10.695 & 12.305 & 8.988 & 11.439 & 13.000 & 8.671 & 10.683 & 12.976 & 8.841 & 3.366 \\ 
AMR & 7.549 & 6.037 & 7.817 & 7.524 & 8.232 & 7.451 & 5.378 & 8.207 & 7.524 & 6.305 & 8.159 & 8.854 \\ 
HT & 9.220 & 7.890 & 9.598 & 9.305 & 9.951 & 9.354 & 8.939 & 9.951 & 9.439 & 9.780 & 9.902 & 7.634 \\ 
HAT & 7.720 & 7.622 & 7.805 & 8.829 & 8.341 & 7.707 & 8.707 & 8.366 & 7.805 & 8.634 & 8.195 & 9.049 \\ 
EFDT & 8.366 & 10.207 & 7.305 & 9.354 & 7.463 & 7.183 & 10.061 & 7.488 & 6.439 & 9.146 & 7.293 & 10.927 \\ 
SGT* & 15.707 & 14.341 & 14.537 & 11.488 & 12.098 & 14.659 & 15.610 & 11.927 & 12.780 & 15.000 & 10.854 & 15.634 \\ 
MT* & 13.159 & 9.037 & 13.622 & 9.256 & 13.841 & 13.232 & 9.232 & 13.915 & 12.890 & 11.890 & 13.256 & 12.524 \\ 
ARF & 6.902 & 5.293 & 7.195 & 8.049 & 7.927 & 6.902 & 5.024 & 7.854 & 7.122 & \textbf{5.244} & 8.293 & 11.024 \\ 
AMF* & 10.744 & 7.524 & 11.159 & 7.207 & 11.695 & 10.866 & 7.037 & 11.671 & 10.695 & 9.085 & 11.232 & 16.110 \\ 
ABALR & 7.195 & \textbf{4.976} & 8.341 & \textbf{6.463} & 8.805 & 7.951 & \textbf{3.512} & 8.805 & 8.732 & 5.488 & 9.098 & 5.683 \\ 
ABOLR & 7.366 & 5.756 & 8.293 & 6.780 & 8.634 & 8.049 & 4.146 & 8.732 & 8.463 & 5.976 & 8.732 & 6.195 \\ 
MLBELS* & 9.268 & 12.829 & 4.610 & 9.024 & 4.220 & 5.293 & 12.073 & 4.341 & 6.317 & 8.902 & 5.659 & 12.195 \\ 
MLHT & 7.756 & 14.415 & 10.024 & 13.537 & 10.098 & 10.854 & 14.561 & 10.293 & 13.049 & 12.585 & 11.049 & \textbf{1.000} \\ 
MLHTPS & 12.329 & 10.390 & 13.354 & 10.427 & 13.402 & 13.634 & 11.683 & 13.476 & 13.390 & 11.488 & 13.329 & 7.854 \\ 
iSOUPT & 7.744 & 5.646 & 8.573 & 6.988 & 8.817 & 8.110 & 4.841 & 8.695 & 8.793 & 6.890 & 9.159 & 4.415 \\ 
\midrule
Friedman's $\chi^{2}$ & 231.48 & 248.68 & 239.21 & 107.07 & 206.71 & 238.17 & 342.55 & 202.84 & 227.82 & 220.85 & 176.03 & 462.72\\
$p$-value & 2.2e-16 & 2.2e-16 & 2.2e-16 & 1.665e-15 & 2.2e-16 & 2.2e-16 & 2.2e-16 & 2.2e-16 & 2.2e-16 & 2.2e-16 & 2.2e-16 & 2.2e-16 \\
\bottomrule
\SetCell[c=13]{l} Best results are in bold.\\
    \end{tblr}
\end{table*}

\begin{figure*}[htb]
    \centering
    \subfloat[Subset Accuracy]{\includegraphics[width=.49\linewidth]{figs/st_subset_acc.pdf}}
    \subfloat[Hamming loss]{\includegraphics[width=.49\linewidth]{figs/st_hamming.pdf}}\\
    \subfloat[Example-based F1]{\includegraphics[width=.49\linewidth]{figs/st_example_f1.pdf}}
    \subfloat[Micro-averaged F1]{\includegraphics[width=.49\linewidth]{figs/st_micro_f1.pdf}}\\
    \subfloat[Macro-averaged F1]{\includegraphics[width=.49\linewidth]{figs/st_macro_f1.pdf}}
    \subfloat[Time (s)]{\includegraphics[width=.49\linewidth]{figs/st_time_s.pdf}}
    
    \caption{Critical distance of Bonferroni-Dunn’s post-hoc tests ($\alpha$ = 99\%)}\label{fig:post-hoc}
\end{figure*}


The results show that MLHAT outperforms on average the other methods in accurate prediction of the labelset of each instance with subset accuracy of 26.46\% as well as the best balance between false positives and false negatives at the instance level (example-based F1 of 47.55\%), and at the label level both absolute (macro F1 of 38.71\%) and prevalence-weighted (micro F1 of 48.55\%). These differences are supported by statistical tests, which indicate that for these metrics MLHAT outperforms the baseline of the Bayesian and rules approaches, \ac{NB} and \ac{AMR}, as well as non-Hoeffding \acp{IDT} \ac{SGT} and \ac{MT}. This indicates that most single-model proposals do not deal well with the additional complexity of \ac{MLC} transformed with \ac{BR} in terms of predicting the exact labelset, the average match by instances, nor the average match by labels. In this line, \acs{MLBELS} and \ac{iSOUPT} obtain better results than these proposals, showing the potential to adapt specific components of the decision tree to the multi-target paradigm. However, they obtain worse results than MLHAT with differences per metric. In the case of \acs{MLBELS}, it is observed that it has problems matching exactly the predicted labelset, although it maintains a good average of hits per label. This makes it significantly worse than MLHAT in subset accuracy, hamming loss, and macro F1, while in Micro F1 and example-based F1, it is at the same level. This may be due to the method used for keeping the co-relation between labels, which is modeled with a neural network. For \ac{iSOUPT}, the results are worse because it does not control the concept drift like \ac{MLHAT} does. This factor also makes \ac{MLHAT} outperform previous Hoeffding trees, although they will be discussed in detail in Section \ref{sec:treescomp}. \ac{kNN} works quite well without the need to explicitly consider the concept drift because it already works with a window of the \textit{n} most recent instances. Finally, ensembles in general also perform better because they combine several classifiers and incorporate concept drift detectors usually. Thus, statistical tests indicate that \ac{MLHAT} only may not differ from \ac{ARF}, \ac{kNN} or \ac{ABA} in different metrics. Although when this occurs, there is no algorithm that excels in more than one metric, so we can state that there is no clear alternative to \ac{MLHAT} in terms of overall accuracy.

However, the results indicate a weakness of MLHAT in terms of the accuracy of the positive labels, that is, it tends to predict an accurate subset of the real labelset, but without including all the active labels. This affects to varying degrees the results in Hamming loss, example-based precision, micro precision, and macro precision, making MLHAT not superior to its most direct competitors, although it is not statistically inferior either. Thus, it can be seen that obtaining a good accuracy across instances, or in other words, minimizing Hamming loss, is a complicated problem, where the performance of the main proposals is blurred. Moreover, good results in this metric do not necessarily imply good subset accuracy. Thus, in this metric, the ensemble-based methods of \ac{ABA} and \ac{ARF} obtain the best results. Attending to example-based precision, MLHAT obtains competitive results against these ensembles. In the label-based approach, the differences are larger and MLHAT is also outperformed by the previous multi-label \ac{IDT} \ac{iSOUPT}. However, we can see that these algorithms obtain these results at the cost of worse recall rates, while MLHAT remains competitive in this metric in all scenarios, making the overall performance in the end superior.

Regarding the real-time factor, the results show that MLHAT is in the middle part of the ranking, close to the \ac{BR}+\ac{HAT} transformation. It is slower than the rest of the multi-label \acp{IDT} and other less sophisticated proposals, such as \ac{NB} or \ac{LR}'s ensembles. On the other hand, it is faster than non-Hoeffding \acp{IDT} \ac{SGT} and \ac{MT}, which have scalability problems for bigger datasets. This is accentuated in the forest approach \ac{AMF}.
MLHAT is also faster than the most similar performing methods: \ac{kNN}, \ac{ARF} and \ac{MLBELS}.
On the one hand, \ac{kNN} is directly dependent on the number of features and the number of instances and, although \ac{MLHAT} also maintains \acp{kNN} in the leaves, the previous partition of the problem with the tree structure considerably accelerates the process. \ac{ARF} is slower because it assembles \acp{HT} in a more computationally demanding system with concept drift detectors at tree level, while \ac{MLHAT} drift detectors operate at branch level, maintaining smaller alternate models. Finally, MLBELS has scalability issues that cause larger datasets to fail. This is due to the combination of an ensemble that maintains as many models as labels, and a mechanism that maintains a pool of discarded models that increases up to 100 per label.
Section \ref{sec:complexcomp} will discuss this factor in more detail in conjunction with the computational complexity and memory consumption evolution of the model.


\begin{table*}[!tb]
    \caption{Results for Micro-averaged F1 on each dataset}\label{tab:datasetf1}
    \begin{tblr}{
        width=\linewidth,
        colspec={Q[l,m] *{17}{X[c,m]}},
        rowsep=-2pt,
        colsep=0pt,
        row{1-Z}={font=\scriptsize},
    }
\toprule
\SetCell[r=2]{} Dataset & MLHAT & &  NB &  & HT &  &  EFDT &  &  MT &  & AMF &  &  ABOLR & & MLHT &   &  iSOUPT &  \\
 &  & KNN & & AMR & & HAT &  &  SGT &  & ARF &  & ABALR &  & MLBELS &  & MLHTPS \\
%Dataset & MLHAT & KNN & NB & AMR & HT & HAT & EFDT & SGT & MT & ARF & AMF & ABALR & ABOLR & MLBELS & MLHT & MLHTPS & iSOUPT \\
\midrule
Flags & 0.586 & 0.642 & 0.642 & 0.575 & \textbf{0.710} & 0.695 & \textbf{0.710} & 0.650 & 0.622 & 0.703 & 0.641 & 0.587 & 0.581 & 0.533 & 0.617 & 0.630 & 0.575 \\
WaterQuality & 0.551 & \textbf{0.561} & 0.549 & 0.552 & 0.420 & 0.436 & 0.459 & 0.352 & 0.357 & 0.533 & 0.509 & 0.549 & 0.553 & 0.465 & 0.258 & 0.382 & 0.547 \\
Emotions & 0.445 & 0.484 & \textbf{0.629} & 0.319 & 0.573 & 0.575 & 0.546 & 0.389 & 0.033 & 0.547 & 0.413 & 0.300 & 0.309 & 0.558 & 0.342 & 0.537 & 0.319 \\
VirusGO & 0.694 & 0.708 & 0.120 & 0.613 & 0.266 & 0.533 & 0.265 & 0.344 & 0.516 & 0.425 & \textbf{0.849} & 0.601 & 0.618 & 0.584 & 0.344 & 0.228 & 0.603 \\
Birds & 0.133 & 0.164 & 0.000 & \textbf{0.176} & 0.000 & 0.000 & 0.122 & 0.081 & 0.065 & 0.115 & 0.108 & 0.174 & 0.154 & 0.156 & 0.000 & 0.000 & 0.175 \\
Yeast & 0.598 & 0.590 & 0.545 & 0.488 & 0.599 & 0.597 & 0.589 & 0.452 & 0.477 & 0.574 & 0.485 & 0.486 & 0.489 & \textbf{0.613} & 0.536 & 0.583 & 0.503 \\
Scene & \textbf{0.936} & 0.803 & 0.579 & 0.908 & 0.502 & 0.591 & 0.715 & 0.269 & 0.651 & 0.817 & 0.845 & 0.905 & 0.904 & 0.783 & 0.187 & 0.604 & 0.879 \\
Gnegative & 0.937 & 0.730 & 0.639 & 0.943 & 0.656 & 0.663 & 0.670 & 0.190 & 0.737 & 0.763 & 0.879 & 0.942 & 0.941 & 0.699 & 0.389 & 0.640 & \textbf{0.945} \\
Plant & 0.770 & 0.319 & 0.309 & \textbf{0.875} & 0.291 & 0.305 & 0.364 & 0.127 & 0.459 & 0.489 & 0.678 & 0.859 & 0.856 & 0.413 & 0.282 & 0.221 & \textbf{0.875} \\
Human & 0.862 & 0.596 & 0.296 & \textbf{0.873} & 0.416 & 0.515 & 0.466 & 0.165 & 0.320 & 0.709 & 0.570 & 0.870 & 0.872 & 0.663 & 0.302 & 0.256 & 0.849 \\
Yelp & \textbf{0.825} & 0.653 & 0.485 & 0.755 & 0.614 & 0.663 & 0.701 & 0.458 & 0.480 & 0.797 & 0.669 & 0.784 & 0.785 & 0.697 & 0.512 & 0.587 & 0.773 \\
Medical & 0.584$^\dag$ & 0.502 & 0.003 & 0.315 & 0.520 & 0.534 & 0.636 & 0.087 & 0.287 & 0.217 & 0.574 & 0.215 & 0.200 & \textbf{0.684} & 0.240 & 0.003 & 0.324 \\
Eukaryote & 0.892 & 0.731 & 0.239 & 0.891 & 0.544 & 0.685 & 0.646 & 0.073 & 0.486 & 0.811 & 0.655 & \textbf{0.898} & 0.897 & 0.776 & 0.270 & 0.242 & 0.876 \\
Slashdot & \textbf{0.458} & 0.156 & 0.000 & 0.030 & 0.106 & 0.172 & 0.244 & 0.064 & 0.012 & 0.140 & 0.260 & 0.013 & 0.010 & 0.417 & 0.142 & 0.009 & 0.074 \\
Enron & 0.436 & 0.374 & 0.436 & 0.499 & 0.429 & 0.431 & 0.442 & 0.129 & 0.303 & 0.448 & 0.451 & 0.510 & 0.511 & \textbf{0.520} & 0.297 & 0.276 & 0.500 \\
Hypercube & 0.993 & 0.994 & 0.963 & 0.982 & 0.917 & 0.962 & 0.931 & 0.028 & 0.995 & 0.993 & \textbf{0.995} & 0.988 & 0.989 & 0.987 & 0.785 & 0.806 & 0.933 \\
Langlog & \textbf{0.133} & 0.074 & 0.000 & 0.054 & 0.000 & 0.000 & 0.099 & 0.015 & 0.011 & 0.003 & 0.012 & 0.035 & 0.036 & 0.127 & 0.002 & 0.048 & 0.061 \\
Stackex & 0.257$^\dag$ & 0.127 & 0.001 & 0.111 & 0.011 & 0.025 & 0.162 & 0.018 & 0.021 & 0.043 & 0.050 & 0.129 & 0.129 & \textbf{0.310} & 0.146 & 0.000 & 0.133 \\
Tmc & 0.638$^\dag$ & 0.487 & 0.322 & 0.618 & 0.529 & 0.525 & 0.463 & 0.325 & 0.424 & 0.516 & 0.503 & 0.629 & 0.621 & \textbf{0.641} & 0.197 & 0.439 & 0.607 \\
Ohsumed & \textbf{0.445} & 0.065 & 0.301 & 0.196 & 0.359 & 0.385 & 0.325 & 0.186 & 0.026 & 0.147 & 0.006 & 0.257 & 0.247 & 0.382 & 0.137 & 0.308 & 0.229 \\
D20ng & \textbf{0.662} & 0.146 & 0.001 & 0.147 & 0.449 & 0.425 & 0.471 & 0.191 & 0.121 & 0.190 & 0.121 & 0.338 & 0.306 & 0.531 & 0.083 & 0.289 & 0.273 \\
Mediamill & \textbf{0.661} & 0.600 & 0.170 & 0.553 & 0.511 & 0.519 & 0.518 & 0.223 & 0.454 & 0.583 & 0.519 & 0.558 & 0.557 & 0.555 & 0.425 & 0.367 & 0.521 \\
Corel5k & 0.284$^\dag$ & 0.138 & 0.018 & 0.025 & 0.078 & 0.141 & 0.134 & 0.010 & 0.153 & \textbf{0.316} & 0.221 & 0.020 & 0.022 & 0.214 & 0.043 & 0.019 & 0.021 \\
Bibtex & \textbf{0.347} & 0.030 & 0.000 & 0.203 & 0.216 & 0.224 & 0.218 & 0.091 & 0.111 & 0.154 & 0.141 & 0.182 & 0.183 & 0.272 & 0.041 & 0.090 & 0.196 \\
Nuswidec & \textbf{0.403} & 0.394 & 0.331 & 0.088 & 0.236 & 0.282 & 0.243 & - & 0.017 & 0.261 & - & 0.075 & 0.075 & - & 0.011 & 0.214 & 0.121 \\
Imdb & 0.226 & 0.169 & 0.187 & 0.025 & 0.047 & 0.054 & 0.085 & 0.006 & 0.000 & 0.033 & - & 0.054 & 0.058 & \textbf{0.353} & 0.242 & 0.013 & 0.038 \\
Nuswideb & \textbf{0.423} & 0.373 & 0.105 & 0.111 & 0.175 & 0.275 & 0.250 & - & - & 0.278 & - & 0.110 & 0.107 & - & 0.010 & 0.109 & 0.119 \\
YahooSociety & 0.435 & 0.232 & 0.349 & 0.394 & 0.243 & 0.290 & 0.250 & - & 0.108 & 0.248 & - & \textbf{0.451} & 0.435 & 0.442 & 0.369 & 0.028 & 0.420 \\
Eurlex & 0.551 & 0.283 & 0.123 & 0.478 & 0.405 & 0.406 & 0.262 & 0.037 & 0.122 & 0.376 & - & \textbf{0.600} & 0.579 & - & 0.074 & 0.021 & 0.546 \\
SynTreeSud & 0.308 & 0.274 & 0.063 & 0.160 & 0.062 & 0.148 & 0.206 & 0.007 & 0.001 & 0.195 & 0.004 & 0.168 & 0.168 & \textbf{0.449} & 0.329 & 0.001 & 0.127 \\
SynRBFSud & 0.292 & 0.251 & 0.209 & 0.222 & 0.294 & 0.351 & 0.257 & 0.008 & 0.040 & \textbf{0.368} & 0.166 & 0.041 & 0.040 & 0.214 & 0.107 & 0.085 & 0.190 \\
SynHPSud & 0.364$^\dag$ & 0.339 & 0.011 & 0.293 & 0.111 & 0.290 & 0.275 & 0.009 & 0.000 & 0.291 & 0.001 & 0.292 & 0.293 & \textbf{0.460} & 0.295 & 0.000 & 0.250 \\
SynTreeGrad & 0.333 & 0.297 & 0.130 & 0.138 & 0.067 & 0.103 & 0.180 & 0.010 & 0.000 & 0.192 & 0.052 & 0.165 & 0.171 & \textbf{0.469} & 0.348 & 0.000 & 0.109 \\
SynRBFGrad & 0.219 & 0.180 & 0.196 & 0.171 & 0.246 & 0.271 & 0.207 & 0.008 & 0.010 & \textbf{0.285} & 0.083 & 0.013 & 0.013 & 0.194 & 0.103 & 0.068 & 0.131 \\
SynHPGrad & 0.324$^\dag$ & 0.279 & 0.058 & 0.183 & 0.089 & 0.162 & 0.211 & 0.007 & 0.000 & 0.185 & 0.011 & 0.166 & 0.165 & \textbf{0.435} & 0.282 & 0.001 & 0.122 \\
SynTreeInc & 0.311 & 0.270 & 0.190 & 0.143 & 0.086 & 0.139 & 0.182 & 0.010 & 0.001 & 0.173 & 0.005 & 0.164 & 0.165 & \textbf{0.443} & 0.316 & 0.000 & 0.105 \\
SynRBFInc & 0.232 & 0.182 & 0.188 & 0.181 & 0.248 & 0.277 & 0.209 & 0.022 & 0.038 & \textbf{0.310} & 0.122 & 0.020 & 0.020 & 0.199 & 0.147 & 0.079 & 0.148 \\
SynHPInc & 0.258 & 0.189 & 0.047 & 0.030 & 0.046 & 0.046 & 0.106 & 0.007 & 0.000 & 0.033 & 0.000 & 0.027 & 0.028 & \textbf{0.393} & 0.291 & 0.000 & 0.036 \\
SynTreeRec & 0.387 & 0.389 & 0.214 & 0.407 & 0.283 & 0.402 & 0.368 & 0.007 & 0.108 & 0.383 & 0.108 & 0.410 & 0.409 & \textbf{0.480} & 0.334 & 0.000 & 0.372 \\
SynRBFRec & 0.242 & 0.193 & 0.216 & 0.243 & 0.352 & \textbf{0.374} & 0.232 & 0.029 & 0.035 & 0.308 & 0.143 & 0.017 & 0.016 & 0.205 & 0.126 & 0.135 & 0.294 \\
SynHPRec & 0.468$^\dag$ & 0.383 & 0.299 & 0.317 & 0.316 & 0.335 & 0.353 & 0.205 & 0.291 & 0.341 & 0.274 & 0.315 & 0.314 & \textbf{0.552} & 0.385 & 0.273 & 0.287 \\
\hline
Average & \textbf{0.486} & 0.374 & 0.248 & 0.373 & 0.318 & 0.361 & 0.360 & 0.139 & 0.222 & 0.373 & 0.337 & 0.364 & 0.362 & 0.470 & 0.252 & 0.210 & 0.371 \\
Ranking & \textbf{3.439} & 6.878 & 11.439 & 7.451 & 9.354 & 7.707 & 7.183 & 14.659 & 13.232 & 6.902 & 10.866 & 7.951 & 8.049 & 5.293 & 10.854 & 13.634 & 8.110\\
\bottomrule
\SetCell[c=18]{l,m,\linewidth} Best results are in bold. $^\dag$ indicates that MLHAT obtains the second best result. \\
\SetCell[c=18]{l,m,\linewidth} Non finished experiments due to scalability problems marked with –. The physical limitations for all the experiments are set to 200GB of RAM and 240 hours of executions.\\
\end{tblr}
\end{table*}


Table \ref{tab:datasetf1} shows the detail of one of the metrics studied, the micro-averaged F1, with the results obtained by each algorithm in each dataset in addition to the average result shown in Table \ref{tab:singleresults} and the ranking of the Table \ref{tab:friedmansingle}. We choose this metric for the detailed analysis for being one of the most balanced in the context of \ac{MLC}, but the detail of the rest of studied metrics have been obtained in the same way and are available in the repository associated. These results confirm that \ac{MLHAT} is not only better on average, but consistently better for datasets with different characteristics, with 10 out of 41 datasets where it is the best and 37 out of 41 in the first quartile. But beyond the comparison, these results serve to identify in which problems \ac{MLHAT} works better and in which it is convenient to use other algorithms. Thus, we can see that for extremely short flows, less than 1000 instances, MLHAT works well in high dimensionality cases such as \textit{Medical} and \textit{VirusGO} where there are more features than instances. If there are not so many features, other simpler models perform better. As other authors discussed \cite{Read2012}, this is due to Hoeffding trees are pretty conservative models that need a lot of instances to grow up. For longer flows, MLHAT generally performs very well, as the tree can grows properly. However, if the number of features is less than 500, ensemble-based methods like \ac{ABA} or \ac{ARF} can obtain better results, as is the case of \textit{Enron}, \textit{Eukaryote}, or \textit{Corel5k}. \ac{MLHAT} performs better than the rest of algorithms in high dimensional spaces probably because of the partitioning of the truly multi-label feature space: by considering label co-occurrence in the decision tree partitioning process, it deals better with the additional complexity of this scenario than transforming the problem or other multi-label decision trees that do not use Bernoulli at this point. On the other hand, keeping two types of classifiers in the leaves makes \ac{MLHAT} remain competitive on streams of all lengths: in shorter cases, \ac{MLHAT}'s behavior will more closely mimic a \ac{kNN}, while in longer ones, it will more closely approximate an \ac{ABA}. 

Synthetic datasets show us that there is a relationship between the distribution of the input data and which algorithms will perform better: streams generated with random tree benefit more from tree-based algorithms, while those generated with \ac{RBF} will be better solved with \ac{NB} or \ac{kNN}, although when working with high dimensionality, ensemble-based methods obtain better results. \ac{MLHAT} works better with Hyper-planes and in general responds better to sudden, gradual and recurrent concept drift. The response of the main methods to different concept drifts will be discussed in detail in Section \ref{sec:driftcomp}.

%Attending to decision tree-based methods, results show that \ac{MLHAT} improves to varying degrees on all other proposals, both Hoeffding-based and non-Hoeffding-based, and both adapted to multi-label learning and transformed. In the category of multi-label Hoeffding trees, Bonferroni-Dumm shows that \ac{MLHAT} is significantly superior to \acs{MLHT} and \acs{MLHTPS} in all metrics. \ac{MLHAT} significally outperforms also Hoeffding-based proposals imported from the multi-class paradigm that do not incorporate concept-drift adaptation, \ac{HT} and \ac{EFDT}. \ac{HAT} obtains slightly better results, but fails mainly in the average accuracy per label. The next section discusses in more detail the causes that make \ac{MLHAT} superior to these previous Hoeffding trees.
%Attending to non-Hoeffding trees, we can see that \acs{iSOUPT} is the \ac{IDT} with the closest performance level to our proposal, which shows the potential of adapting specific components of the decision tree to the multi-target paradigm, as opposed to transforming the problem and applying multi-class methods. However, \ac{MLHAT} outperforms significantly \acs{iSOUPT} in terms of macro-averaged F1. It is also observed that the other recent non-Hoeffding-based \acp{IDT} transformed from multi-class learning, \acs{SGT} and \acs{MT}, are significantly lower than \ac{MLHAT}, which indicates that they do not deal well with the additional complexity of \ac{MLC} in terms of predicting the exact labelset, the average match by instances, and also the average match by labels.

%Finally, we compare \acs{MLHAT} with ensemble-based models, both based on forests, \acs{ARF} and \acs{AMF}, and with concept drift detection, \acs{ABA} and \acs{ABO}. These methods have smaller differences with \ac{MLHAT} because they combine the predictive power of more than one classifier in systems that are also more computationally demanding and slower in processing stream instances. More specifically, \acs{ABA} and \acs{ABO}, have closer performance attending to all \ac{MLC} indicators, probably due to the concept detection. \acs{MLHAT} also incorporates this mechanism, but also a more potent classifier, which makes possible a higher performance without having to use an ensemble architecture. In the case of \acs{ARF} and \acs{AMF}, they are close to being statistically worse than \acs{MLHAT}. This is due to their base classifier, \ac{HT} and \acs{MT}, weak \acp{IDT} that have already been shown not to capture well the particularities of \ac{MLC}.





\subsection{Analysis of MLHAT compared to previous Hoeffding trees}\label{sec:treescomp}

After comparing \ac{MLHAT} with all other online \ac{MLC} paradigms, the second study addresses RQ2 by focusing the comparison on previous Hoeffding \acp{IDT} and specifically \ac{HAT}, an algorithm with several common elements with \ac{MLHAT} but ignoring the additional complexity of multi-label learning. For this analysis, Tables \ref{tab:singleresults}, \ref{tab:friedmansingle}, and \ref{tab:datasetf1}, and Figure \ref{fig:post-hoc} previously discussed are analyzed putting the focus in the Hoeffding trees.

As has been shown in the previous section, \acs{MLHAT} is $8.9\%$ better at predicting the exact labelset for an instance than the transformation \ac{BR}+\ac{HAT}, and around $20\%$ in the different versions of the F1 score, indicating better accuracy per label. This differences are confirmed by Bonferroni-Dunn, that indicates superiority of \ac{MLHAT} in all the metrics except for Hamming loss and the time of execution, in which they are equivalent.
This implies that introducing a natively multi-label split criterion that takes into account label co-occurrence through a multi-variate Bernoulli distribution is a more effective approach than trying to classify each label separately with \ac{BR}+\ac{HAT}. In addition, considering this occurrence allows our model to adapt itself to the label imbalance that affects the number of labels that each leaf separates, which also contributes to increase the benefits of \ac{MLHAT} over \ac{HAT}. Synthetic datasets with explicit concept drift information show in general that \ac{MLHAT} is more responsive to different types of concept drift than HAT. This means that, although both have \ac{ADWIN}-based branch-level detectors, \ac{MLHAT}'s approach of considering all labels together obtains better results than considering the accuracy of each label individually. However, as the \ac{RBF} generator-based datasets indicate, the HAT drift detector may perform better with data following this distribution. Finally, in terms of execution time, \ac{MLHAT} is 2.7 times faster than \ac{HAT} on average. This is due to the fact that in \ac{BR} a tree must be maintained for each label, which is slower than maintaining a single tree, even though it has extra computational load due to the leaves classifiers.

\ac{HT} and \ac{EFDT} are Hoeffding trees that have the same problems as \ac{HAT} due to not adapting the algorithm to the multi-label context, in addition to slightly worsening the results by not incorporating concept drift detection. In particular, the way of applying the Hoeffding bound "with less guarantees" of \ac{EFDT} versus \ac{HT} seems to benefit it more, since it compensates the absence of drift adaptation with a faster tree growth method. \ac{MLHAT} applies the Hoeffding bound more similarly to \ac{HT} and \ac{HAT}, although the other modifications and components specific to the multi-label problem have more effect on the performance of the algorithm, so it obtains better results than \ac{EFDT}, and also than \ac{HT}, in all the criteria.

Attending to previous Hoeffding trees adaptations to \ac{MLC}, \ac{MLHT} and \ac{MLHTPS}, the results show that \ac{MLHAT} outperform them in all the performance metrics. In these cases we observe how the results penalize a partitioning criterion that does not consider the co-occurrence of labels, as well as the absence of concept drift adaptation. Thus, we see that only a multi-label classifier on the leaves is not enough to obtain competitive results. In this line, it can be extracted from the results in Table \ref{tab:datasetf1} that in general the more complex \ac{MLHTPS} leaf classifier is more beneficial, although the exception is the synthetic data generated with Random Tree, where the technique of predicting the majority labelset in each \ac{MLHT} leaf is preferable. In these cases it even outperforms our \ac{MLHAT}. However, in light of the general trend, it is worth asking whether this generator, despite being widely used in the literature, provides realistic data, since their results are quite different from other synthetic results and especially from real-world datasets. On the other hand, the differences in execution times of \ac{MLHT} and \ac{MLHTPS} allow us to quantify how influential the leaf classifier is on the real-time factor in these models. Thus, we can see that, while \ac{MLHT} is the fastest model in the experiment, the change from the base classifier to an expensive model such as the Prune Set ensemble of \acp{HT} increases the execution time by about 20 times on average. This gives us an idea of the importance of the classifiers in \ac{MLHAT} for the complexity of the model. Thus, the \ac{MLHAT} time metrics show that in this sense it is more beneficial to maintain two less computationally expensive classifiers such as \ac{kNN} and \ac{ABA}+\ac{LR} for each leaf.



%\subsection{Ensembles comparison}

%The second experiment focuses on the ensemble-based models to study the potential of our \acs{MLHAT} in this paradigm, as was introduced in RQ3. Due to the computational cost of some tree-based ensembles, this study excludes the more complex \textcolor{red}{7} datasets. Specifically, it focuses on the \textit{Flags} to \textcolor{red}{\textit{Corel16k}} datasets from Table \ref{tab:datasets}, which still compose a set of \textcolor{red}{29} different experiments per algorithm to draw meaningful conclusions. Table \ref{tab:ensembleresults} shows a summary of the results by averaging the measures for the selected datasets, while Table \ref{tab:ensemblesubacc} breaks down the subset accuracy measures by algorithm against each dataset. The complete results are available in the repository \textcolor{red}{[REP]}. It can be observed that ensembles using \acs{MLHAT} as base classifier achieve the best average result for most of the metrics, with the random sub-spaces method, \acs{SRPMLHAT}, as the superior one. However, in this case there are less difference among results, with other promising algorithms also based on random sub-spaces like \acs{SRPiSOUPT}.


%Based on these results, statistical tests on main metrics are carried out to find significant differences. Friedman test and post-hoc Bonferroni-Dunn procedure \cite{Dietterich1998} are applied to evaluate the differences across all dataset in subset accuracy, example-based F1, macro-averaged F1 and micro-averaged F1. Table \ref{tab:friedmanensemble} presents the ranks assigned by Friedman's test as well as the obtained $p$-value. Figures \ref{fig:bdensemblesubacc} to \ref{fig:bdensemblemicf1} show the results of Bonferroni-Dunn for metrics with significant differences at confidence level $\alpha=99\%$. There are significant differences with high confidence ($p\mathrm{-value} \rightarrow 0$) for all the metrics. These differences are mostly centered on ensemble versions of previos multi-label adaptations, like \acs{OBiSOUPT}, \acs{OBMLHTPS} or \acs{SRPMLHTPS}, and binary relevance adaptations of models without concept-drift detection, like \acs{OBHT} or \acs{AMF}. It can be observed that \acs{SRPHAT}  and \acs{OBMLHAT} have fairly equal performances, especially in subset accuracy, but with the extra burden of the random subspacing of \acs{SRPHAT}. When this additional preprocessing is introduced also in MLHAT ensemble, \acs{SRPMLHAT} consistently obtains the best results.



\subsection{Analysis of concept drift adaptation}\label{sec:driftcomp}

This section addresses RQ3 by making a detailed analysis of the evolution of \ac{MLHAT} performance along the data stream and how it responds to different concept drift in both real and synthetic scenarios. To facilitate the presentation of results, this section focuses the comparative study on the most competitive algorithms according to the results of Section \ref{sec:overallperf} and trying to include only one representative in the case of families with more than one algorithm. Thus, \ac{HAT}, \ac{kNN}, and \ac{AMR} are included as the most competitive \ac{BR} transformations of single models; \ac{ABA} and \ac{ARF} represent the \ac{BR} transformations of ensembles; and \acs{MLBELS}, \ac{MLHT}, and \ac{iSOUPT} cover the previous \ac{AA}.

\begin{figure*}[!tb]
    \centering
    \subfloat[Yelp]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_Yelp.pdf}}
    \subfloat[Ohsumed]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_Ohsumed.pdf}}
    \subfloat[D20ng]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_D20ng.pdf}}
    \subfloat[Nuswideb]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_Nuswideb.pdf}}\\
    
    \subfloat[SynHPSud]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynHPSud.pdf}}
    \subfloat[SynTreeGrad]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynTreeGrad.pdf}}
    \subfloat[SynRBFInc]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynRBFInc.pdf}}
    \subfloat[SynRBFRec]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynRBFRec.pdf}}\\

    \subfloat[SynRBFSud]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynRBFSud.pdf}}
    \subfloat[SynHPGrad]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynHPGrad.pdf}}
    \subfloat[SynTreeInc]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynTreeInc.pdf}}
    \subfloat[SynHPRec]{\includegraphics[width=.248\linewidth]{figs/paper_evolmicrof1_SynHPRec.pdf}}
    
    \caption{Prequential evaluation on a selection of datasets with concept drift (expressed as vertical lines). The type of concept drift is given by the name of the synthetic dataset; more information in Table \ref{tab:datasets-synth}.}
    \label{fig:prequential}
\end{figure*}


Figure \ref{fig:prequential} shows the evolution of the micro-averaged F1 score on a subset of the studied datasets that have a temporal order and different types of concept drift. The complete relation of datasets and the rest of metrics are available in the repository associated to the work\footnote{\url{https://github.com/aestebant/mlhat}}. These results show great variability and that there is no one algorithm that fits all data distributions without exception. It can be extracted that \ac{kNN} is characterized by having an acceptable performance from early stages of the stream and being resistant to class imbalance and concept changes. However, the high dimensionality and the impossibility to remember past features make it stagnate compared to other models like \ac{HAT} or \ac{ARF}, as can be seen in \textit{D20ng} or \textit{Yelp}. Models that in different ways are based on cooperation of linear models, \ac{AMR}, \ac{ABA}, and \ac{iSOUPT}, follow similar patterns: they perform better after having seen large number of instances and gradual concept changes as in \textit{Yelp} or \textit{SynHPGrad}. \ac{MLHAT} in a way evolves on these two approaches thanks to the synergy of its two base classifiers: at the beginning of the stream it improves rapidly thanks to the \acp{kNN} it uses as low complexity leaf classifiers. Later on, if the complexity increases, the \ac{LR} baggings, improved by the built tree structure, take part in this scenario. This is seen in \textit{D20ng} or \textit{SynHPRec}. This contrasts with the rest of Hoeffding trees, that need more number of instances to grow and obtain good results. Thus, we see that \ac{MLHAT} performs better than the \ac{MLHT} and \ac{MLHTPS} adaptations probably because the latter do not adapt the partitioning criterion to label co-occurrence and do not have concept drift detector. \ac{MLHT} may perform better on synthetic tree-based data, but its performance declines when concept drift appears as seen in \textit{SynTreeInc} and \textit{SynHPRec}. On the other hand, \ac{ARF} and \ac{HAT}, the \ac{BR} transformations of Hoeffding trees, may perform better than \textit{MLHAT} on data generated with \ac{RBF}, although they are not perfect in these scenarios either as they do not perform uniformly for all distributions through which the stream passes. This may be due to the greater complexity of this data and the greater number of labels, which makes the \ac{BR} ensemble necessary, and even more so if it is a forest ensemble as is the case with \ac{ARF}. Finally, MLBELS depends very much on the type of stream. In general, it responds well to different types of concept drift in Hyperplane and RandomTree, while in real data and \ac{RBF}, although it maintains stable performance, the nature of the neural networks it works with does not allow it to learn more complex patterns well.

By concept drift type, \ac{MLHAT} is the proposal that offers the most uniform performance across the different types. The robustness and uniformity in performance in all cases stands out: there may be models that obtain better results in sections of the stream, but \ac{MLHAT} resists better the concept changes in the sudden, gradual and, especially, recurrent cases as we see in \textit{SynHPRec} and \textit{SynTreeRec}. This indicates that it is highly beneficial to use a multi-label metric to monitor concept drift, as it detects changes more quickly than the alternatives, which monitor each label separately. This flexibility in the face of different types of concept drift makes \ac{MLHAT} stand out especially in real datasets, which have more mixed concept drift patterns.
The incremental concept drift is the most complicated for all algorithms and \ac{MLHAT} is not an exception. We see how in \textit{SynHPInc} it is outperformed by \ac{MLHT} and and \acs{MLBELS}, and in \textit{SynRBFInc} by \ac{ARF} \ac{HAT} and \ac{kNN}. In these cases it might be worth exploring an ensemble option. Hamming loss is the metric used in the experimentation for detecting the concept drift in MLHAT, for serving well in general for all the types of concept drifts, especially those found in real datasets (see Section \ref{sec:optimization}). Hoever, perhaps if one wanted to maximize adaptability to abrupt change, it would be more beneficial to employ another metric such as subset accuracy.


%These results show that \acs{MLHAT} can be solidly better than the rest of tree-based proposals, including those based on ensembles, attending both to predicting the exact labelset for each instance and to the performance across the different labels. This superiority is seen from the beginning of the data flow, where good results are achieved more quickly, demonstrating the usefulness of the leaf classifier for low cardinality. As the flow progresses and concept drift appears, most simple algorithms have steep performance drops, while in the case of \acs{MLHAT} it drops less and recovers sooner. Especially noteworthy is the improvement over the previous \acs{HAT} proposal, which performs especially poorly on datasets such as \textit{Scene}, with many labels and highly correlated with each other. It can be seen that \acs{iSOUPT} (the most recent \ac{IDT} adaptation to multi-label) and \acs{AMF} and \acs{ARF} (the forest ensembles) have a performance most similar to our proposal. However, there are features that make some of these models not robust to all scenarios: the high cardinality in \textit{Mediamill} affects \acs{iSOUPT}, the high density in a short stream of \textit{Scene} affects both \acs{iSOUPT} and \acs{ARF} and the high number of features in \textit{Tmc} affects \acs{AMF}. On the contrary, \ac{MLHAT} performs well in all these scenarios.

%However, \ac{MLHAT} does not perform equally well in all datasets. We have observed that in datasets with high density and short duration of the stream, such as \textit{Flags}, \textit{Emotions}, \textit{Birds} or \textit{WaterQuality}. Figure \ref{fig:preqwaterquality} shows a representative example of this case. It can be seen how in these cases it is more difficult to be accurate in the labelset to be predicted, with a worse subset accuracy and hamming loss. However, an acceptable performance is still maintained considering the success ratio per label, as indicated by the F1 measures around 55\%. In these cases the best methods are forest-based, which seems to indicate that an ensemble system for \ac{MLHAT} could overcome the difficulties encountered with these highly dense datasets, as these models can split the feature space to find the most relevant attributes for each label. 

%ESTE ES EL CASO DE SCENE DONDE HEMOS DICHO QUE NO AFECTA, REVISAR LA CASUÍSTICA
%However, in this detailed study by dataset, we also find a \ac{MLHAT} limitation. We have observed that in datasets with high density and short duration of the stream, such as \textit{Flags}, \textit{Emotions}, \textit{Birds}, or \textit{WaterQuality}, \ac{MLHAT} loses performance. Figure \ref{fig:preqwaterquality} shows a representative example of this case. It can be seen how in these cases it is more difficult to be accurate in the labelset to be predicted, with a worse subset accuracy and hamming loss. However, acceptable performance is still maintained considering the success ratio per label, as indicated by the F1 measures around 55\%. In these cases, the best methods are forest-based, which seems to indicate that an ensemble system for \ac{MLHAT} could overcome the difficulties encountered with these highly dense datasets, as these models can split the feature space to find the most relevant attributes for each label.


%Looking at ensemble-based models, they tend to improve on their corresponding simple model when concept drift appears. This improvement is not so marked in \acs{SRPMLHAT} with respect to \acs{MLHAT}, which already outperforms other ensembles in simpler datasets. However, in more complex datasets and with a greater number of labels, it is observed that the promotion of diversity in instance and feature spaces of \acs{SRPMLHAT} achieves a better initial performance that is maintained throughout the data stream.


\subsection{Analysis of efficiency}\label{sec:complexcomp}

In the context of data stream classification, the efficiency and speed of processing the instances is of great importance, as they are expected to arrive at high speed. Thus, the model must not only be accurate, it must also be scalable and keep its growth controlled over time. It has been shown in the study of Section \ref{sec:overallperf} that \ac{MLHAT} is a time competitive algorithm. In this section we analyze  the detail of the time and memory consumption of \ac{MLHAT}.

The space and time complexity of \ac{MLHAT} are upper-bounded by \ac{HT} and lower-bounded by the \ac{ADWIN} method to prune nodes. Thus, following the reasoning of \cite{Garcia-Martin2021}, we can divide the operations on the tree into three main components: updating the statistics at the leaf, evaluating possible splits, and the learning in the corresponding leaf classifier. Updating the statistics requires traversing the tree to the leaf and updating the label counts at each node along the path. This has a complexity of $O(hl)$ where $h$ is the height of the tree and $l$ is the number of labels in the multi-label problem. To look for possible splits, $f$ splits will be evaluated, where $f$ is the number of features or attributes. For each $f$ split, $v$ computations of information gains are required. Finally, each information gain requires $c$ operations. Thus, split evaluations require $O(fvc)$ operations. Lastly, the complexity of learning in the leaves is upper bounded by the high complexity classifier, a bagging method that aggregates $k=10$ logistic regressions, whose complexity depends mainly on the number of features $f$. Thus, this step has a complexity of $O(kf)$. In conclusion, the total complexity of \ac{MLHAT} in the worst case scenario will be $O(hlf^2vck)$. Empirical results are shown below to observe the real resource consumption of \ac{MLHAT} and how the concept drift affects it.

\begin{figure*}[!tb]
    \centering
    \subfloat[Yelp time]{\includegraphics[width=.248\linewidth]{figs/paper_evoltime_Yelp.pdf}}
    \subfloat[D20ng time]{\includegraphics[width=.248\linewidth]{figs/paper_evoltime_D20ng.pdf}}
    \subfloat[SynRBFSud time]{\includegraphics[width=.248\linewidth]{figs/paper_evoltime_SynRBFSud.pdf}}
    \subfloat[SynHPGrad time]{\includegraphics[width=.248\linewidth]{figs/paper_evoltime_SynHPGrad.pdf}}\\
    \subfloat[Yelp memory]{\includegraphics[width=.248\linewidth]{figs/paper_evolmb_Yelp.pdf}}
    \subfloat[D20ng memory]{\includegraphics[width=.248\linewidth]{figs/paper_evolmb_D20ng.pdf}}
    \subfloat[SynRBFSud memory]{\includegraphics[width=.248\linewidth]{figs/paper_evolmb_SynRBFSud.pdf}}
    \subfloat[SynHPGrad memory]{\includegraphics[width=.248\linewidth]{figs/paper_evolmb_SynHPGrad.pdf}}
    
    \caption{Resources consumption on a selection of the biggest datasets using logarithmic scale}
    \label{fig:resources}
\end{figure*}

Figure \ref{fig:resources} shows the evolution in time and memory consumption of the different paradigms for a selection of datasets that combine the largest number of instances and different number of attributes. To facilitate the visualization of results, only the most representative methods selected in the previous section are plotted here. The results show that \ac{MLHAT} is faster and more efficient than most models, specially models of similar performance like \ac{kNN} and \ac{MLBELS}. This has a lot to do with the use of a single decision tree and the concept drift adaptation. Thus, when this concept drift is detected and the pruning of some of the obsolescent parts of the tree occurs, the memory occupied by the model decreases, which also affects the processing speed of the instances. In contrast, other \ac{IDT}-based models such as \ac{MLHTPS}, \ac{iSOUPT}, \ac{SGT} or \ac{AMF} grow without limit, which can be problematic for longer streams. This is the case for \ac{SGT} and \ac{AMF} in \textit{Nuswideb} for example. Their results have not been able to finish due to requiring hundreds of GB of RAM and/or more than 240 hours of execution. Other models based on HT and with concept drift such as \ac{ARF} and \ac{HAT} also scale poorly, especially with datasets with many labels. This is due to the multi-label transformation of \ac{BR} requires training one model for each label. In the case of \ac{ARF}, this implies a memory consumption that can be 100 times higher than that of \ac{MLHAT} and takes 10 times longer to process the same amount of information. Other proposals such as \ac{kNN} or \ac{ABA} imply minimal or no building of the model which makes them very efficient in memory and also in time. \ac{MLHAT} builds its leaf classifiers on these models, so the presence of them hardly affects the total computation of time and memory used by our proposal, keeping it competitive with other tree-based models like \ac{MLHTPS} or \ac{iSOUPT}.


